Building Vision Models upon Heat Conduction

Visual representation models leveraging attention mechanisms are challenged by significant computational overhead, particularly when pursuing large receptive fields. In this study, we aim to mitigate this challenge by introducing the Heat Conduction Operator (HCO) built upon the physical heat conduction principle. HCO conceptualizes image patches as heat sources and models their correlations through adaptive thermal energy diffusion, enabling robust visual representations. HCO enjoys a computational complexity of O(N^1.5), as it can be implemented using discrete cosine transformation (DCT) operations. HCO is plug-and-play, combining with deep learning backbones produces visual representation models (termed vHeat) with global receptive fields. Experiments across vision tasks demonstrate that, beyond the stronger performance, vHeat achieves up to a 3x throughput, 80% less GPU memory allocation, and 35% fewer computational FLOPs compared to the Swin-Transformer. Code is available at https://github.com/MzeroMiko/vHeat.

==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

%We introduce vHeat, a visual representation model that combines the benefits of global receptive fields, computational efficiency, and enhanced interpretability. The effectiveness of the vHeat model family, including vHeat-T/S/B models, has been demonstrated through extensive experiments and ablation studies, significantly outperforming popular CNNs and ViTs. The results highlight the potential of vHeat as a new paradigm for vision representation learning, offering fresh insights for the development of physics-inspired visual representation models.
%
We introduce vHeat, a visual representation model that integrates the advantages of global receptive fields, computational efficiency, and enhanced interpretability. Extensive experiments and ablation studies demonstrate the efficiency and effectiveness of the vHeat model family, including vHeat-T/S/B models, which significantly outperform popular CNNs and ViTs. These results highlight vHeat's potential as a novel paradigm for vision representation learning, offering fresh insights for the development of physics-inspired representation models in computer vision.
